WAIC, but Why? Generative Ensembles for Robust Anomaly Detection

Machine learning models encounter Out-of-Distribution (OoD) errors when the data seen at test time are generated from a different stochastic generator than the one used to generate the training data. One proposal to scale OoD detection to high-dimensional data is to learn a tractable likelihood approximation of the training distribution, and use it to reject unlikely inputs. However, likelihood models on natural data are themselves susceptible to OoD errors, and even assign large likelihoods to samples from other datasets. To mitigate this problem, we propose Generative Ensembles, which robustify density-based OoD detection by way of estimating epistemic uncertainty of the likelihood model. We present a puzzling observation in need of an explanation -- although likelihood measures cannot account for the typical set of a distribution, and therefore should not be suitable on their own for OoD detection, WAIC performs surprisingly well in practice.

==> supplemental_rate.tex <==
\section{OoD detection with Rate Terms}

Rate is $\KL ( q_\theta(z|x) \Vert p(z) )$ term in the VAE objective. It represents information loss between encoder distribution and prior over latent code.  Table~\ref{table:supplemental_results_table} shows that rate is a powerful classifier variable in OoD detection. For Fashion MNIST, the same $\beta$-VAE model as the ones for Table 1 of the original paper are used. 

==> supplemental_sensitivity.tex <==
\section{Robustness to Perturbations}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/downscaledMNIST.png}
  \caption{Sensitivity to perturbations. Left: VAE assigns higher IWAE values to scaled-down MNIST (red) than to original MNIST (blue). Starting from a scale of .4, each scale increment corresponds to an image scale by 2.5\%. The red and blue line represent average IWAE over 1000 scaled and original MNIST samples, resp. They intersect at the point where the scale is 100\%. IWAE plummets on scaled-up MNIST. Right: Red histogram corresponds to IWAE on scaled-down MNIST by a scale of .4 and the blue one on original MNIST}
  \label{fig:single_model_failure}
\end{figure}


==> supplemental_waic.tex <==
\section{WAIC}

A principle problem in modelling is attempting to estimate expectations under the true data distribution, as distinct from expectations estimated from the training set.  \emph{Information criteria} offer a means for estimating the difference~\cite{gelman}. In this work we utilize the \emph{Watanabe Akaike Information Criteria}~\cite{watanabe2010asymptotic}, which gives an asymptotically correct estimate.  For completeness, we give a short derivation here following the style and form of \citet{watanabegreen}. 


==> tables/corruption_results.tex <==

\begin{table}[h]
  \caption{AUROC of our models on indistribution samples corrupted by 19 different corruption types}
  \label{table:corruption_results_table}
  \centering
  \begin{tabular}{lllllll}
    \toprule
Train Dataset & Corruptions & $D$ & Var($D$) & Rate & $\log p_\theta(\rx)$ & WAIC \\
    \midrule % trained on MNIST
 MNIST & Gaussian Noise & 81.6 & 95.4 & 42.5 & 100 & 100 \\
       & Shot Noise & 44.7 & 80.2 & 46.1 & 61.1 & 59.8 \\
       & Impulse Noise & 80.1 & 53.8 & 52.4 & 99.9 & 99.6 \\
       & Defocus Blur & 96.5 & 100 & 57.7 & 100 & 99.9 \\ 
       & Glass Blur & 100 & 100 & 70.0 & 99.8 & 99.6 \\
       & Motion Blur & 99.5 & 100 & 74.2 & 99.9 & 99.7 \\
       & Zoom Blur & 100 & 99.9 & 49.2 & 94.1 & 92.8 \\
       & Snow & 92.0 & 100 & 55.7 & 100 & 100 \\
       & Frost & 99.9 & 100 & 61.0 & 100 & 100 \\
       & Fog & 99.6 & 100 & 70.2 & 100 & 100 \\
       & Brightness & 85.9 & 100 & 41.4 & 100 & 100 \\
       & Contrast & 97.6 & 100 & 53.9 & 100 & 100 \\
       & Elastic Transform & 99.9 & 99.5 & 80.8 & 96.3 & 96.1 \\
       & Pixelate & 4.42 & 99.3 & 59.5 & 89.8 & 88.2 \\
       & JPEG compression & 99.5 & 91.7 & 42.9 & 96.3 & 95.3 \\
       & Speckle Noise & 45.8 & 83.9 & 45.7 & 62.7 & 61.2 \\
       & Gaussian Blur & 100 & 100 & 41.3 & 98.8 & 98.3 \\
       & Spatter & 64.6 & 70.3 & 53.4 & 95.3 & 98.0 \\
       & Saturate & 50.0 & 50.0 & 49.9 & 50.0 & 50.0 \\
    \midrule % trained on Fashion MNIST
Fashion MNIST & Gaussian Noise & 97.0 & 76.0 & 68.8 & 87.8 & 90.6 \\
       & Shot Noise & 73.3 & 49.0 & 49.3 & 51.2 & 51.2 \\
       & Impulse Noise & 80.7 & 63.9 & 74.0 & 73.7 & 76.7 \\
       & Defocus Blur & 99.7 & 93.9 & 67.9 & 79.9 & 80.0 \\ 
       & Glass Blur & 99.9 & 72.2 & 71.9 & 74.8 & 75.2 \\
       & Motion Blur & 99.0 & 76.0 & 84.8 & 78.5 & 79.1 \\
       & Zoom Blur & 96.1 & 59.1 & 58.2 & 67.6 & 67.8 \\
       & Snow & 79.1 & 88.1 & 91.9 & 97.9 & 99.4 \\
       & Frost & 76.2 & 97.8 & 92.6 & 99.2 & 99.8 \\
       & Fog & 87.2 & 99.9 & 85.3 & 100 & 100 \\
       & Brightness & 62.9 & 88.8 & 88.1 & 98.5 & 99.5 \\
       & Contrast & 86.9 & 98.6 & 80.3 & 96.6 & 98.4 \\
       & Elastic Transform & 95.0 & 60.6 & 88.1 & 74.6 & 78.4 \\
       & Pixelate & 26.7 & 79.8 & 51.7 & 64.7 & 65.2 \\
       & JPEG compression & 96.1 & 66.6 & 51.8 & 63.0 & 63.2 \\
       & Speckle Noise & 72.3 & 49.1 & 49.0 & 51.4 & 51.3 \\
       & Gaussian Blur & 99.6 & 77.2 & 53.1 & 70.9 & 70.7 \\
       & Spatter & 68.8 & 58.4 & 75.2 & 75.8 & 80.5 \\
       & Saturate & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\
    \midrule % trained on Cifar10
 CIFAR-10 & Gaussian Noise & 94.8 & 98.5 & N/A & N/A & N/A \\
       & Shot Noise & 94.2 & 98.5 & N/A & N/A & N/A \\
       & Impulse Noise & 96.2 & 99.3 & N/A & N/A & N/A \\
       & Defocus Blur & 66.3 & 58.0 & N/A & N/A & N/A \\
       & Glass Blur & 68.0 & 51.0 & N/A & N/A & N/A \\
       & Motion Blur & 61.8 & 48.9 & N/A & N/A & N/A \\
       & Zoom Blur & 56.8 & 48.8 & N/A & N/A & N/A \\
       & Snow & 48.9 & 55.5 & N/A & N/A & N/A \\
       & Frost & 55.1 & 56.6 & N/A & N/A & N/A \\
       & Fog & 78.2 & 54.8 & N/A & N/A & N/A \\
       & Brightness & 49.4 & 54.8 & N/A & N/A & N/A \\
       & Contrast & 73.3 & 44.7 & N/A & N/A & N/A \\
       & Elastic Transform & 59.1 & 47.7 & N/A & N/A & N/A \\
       & Pixelate & 58.5 & 47.6 & N/A & N/A & N/A \\
       & JPEG compression & 69.8 & 44.6 & N/A & N/A & N/A \\
       & Speckle Noise & 93.5 & 97.3 & N/A & N/A & N/A \\
       & Gaussian Blur & 57.7 & 55.5 & N/A & N/A & N/A \\
       & Spatter & N/A & N/A & N/A & N/A & N/A \\
       & Saturate & 39.7 & 48.1 & N/A & N/A & N/A \\
    \bottomrule
 \end{tabular}
\end{table}


==> tables/icml_table.tex <==
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> tables/related_work_table.tex <==

\newcommand{\rA}{
  & Auxiliary ``Other'' class & Binary classification (likelihood ratio) \\ 
  &                                     & Adversarial Training
}

\newcommand{\rB}{
   & \cite{hendrycks2016baseline} &  Density Estimation \\ 
   & \cite{gal2016dropout} & Generative Ensembles (ours) \\
   & \cite{liang2017enhancing} &  \\
   & \cite{lakshminarayanan2017simple} &  \\
   & \cite{alemi2018uncertainty} & \\
}

\begin{table}[h]
 \caption{Categorization of several OoD detection techniques, based on whether they depend on a specific model/task, and whether they assume a specific anomaly distribution.}
\label{table:related_table}
\centering
\begin{tabular}{llll}
\toprule
    &Model-Dependent  &Model-Independent \\
\midrule
\multirow{2}{2cm}{OoD Dependent} \rA \\
\midrule
\multirow{2}{2cm}{OoD Independent} \rB \\
\bottomrule
 \end{tabular}
\end{table}


% \begin{table}[ht]
% \caption{Multi-row table}
% \begin{center}
% \begin{tabular}{cc}
%     \hline
%     \multirow{2}{*}{Multirow}&X\\
%     &X\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:multicol}
% \end{table}


